Large-scale Hierarchical Alignment for Data-driven Text Rewriting

We propose a simple unsupervised method for extracting pseudo-parallel monolingual sentence pairs from comparable corpora representative of two different text styles, such as news articles and scientific papers. Our approach does not require a seed parallel corpus, but instead relies solely on hierarchical search over pre-trained embeddings of documents and sentences. We demonstrate the effectiveness of our method through automatic and extrinsic evaluation on text simplification from the normal to the Simple Wikipedia. We show that pseudo-parallel sentences extracted with our method not only supplement existing parallel data, but can even lead to competitive performance on their own.

==> tables/pseudo-dataset-table.tex <==
\begin{table*}[]
\small
\centering
\caption{\small{Datasets used to extract pseudo-parallel monolingual sentence pairs in our style transfer experiments.}}
\label{table:datasets}
\begin{tabular}{c|c|c|c|c|c|c}
\hlineB{3}
\textbf{Dataset} & \textbf{Type} & \textbf{Documents} & \textbf{Tokens} & \textbf{Sentences} & \textbf{Tok. per sent.} & \textbf{Sent. per doc.} \\ \hlineB{3}
PubMed & Scientific papers & 1.5M & 5.5B & 230M & 24 $\pm$ 14 & 180 $\pm$ 98 \\ %\hline
MEDLINE & Scientific abstracts & 16.8M & 2.6B & 118M & 26 $\pm$ 13 & 7 $\pm$ 4 \\ %\hline
EurekAlert & Press releases & 358K & 206M & 8M & 29 $\pm$ 15 & 23 $\pm$ 13 \\ \hlineB{3}
\end{tabular}
\end{table*}
